I-Con: A Unifying Framework for Representation Learning

As the field of representation learning grows, there has been a proliferation of different loss functions to solve different classes of problems. We introduce a single information-theoretic equation that generalizes a large collection of modern loss functions in machine learning. In particular, we introduce a framework that shows that several broad classes of machine learning methods are precisely minimizing an integrated KL divergence between two conditional distributions: the supervisory and learned representations. This viewpoint exposes a hidden information geometry underlying clustering, spectral methods, dimensionality reduction, contrastive learning, and supervised learning. This framework enables the development of new loss functions by combining successful techniques from across the literature. We not only present a wide array of proofs, connecting over 23 different approaches, but we also leverage these theoretical results to create state-of-the-art unsupervised image classifiers that achieve a +8% improvement over the prior state-of-the-art on unsupervised classification on ImageNet-1K. We also demonstrate that I-Con can be used to derive principled debiasing methods which improve contrastive representation learners.

==> sections/table-orig.tex <==


\begin{table}[p]
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1.5} % Adjusts the row spacing
    \setlength{\tabcolsep}{8pt} % Adjusts column spacing

    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|>{\centering\arraybackslash}p{2.7cm}|>{\centering\arraybackslash}p{5.8cm}|>{\centering\arraybackslash}p{5.9cm}|} 
        \rowcolor{lightgray!50} % Header background color
        \hline\textbf{Method} & \textbf{Choice of $p_\theta(j|i)$} & \textbf{Choice of $q_\phi(j|i)$} \\ [2pt] % Adds a small space after the header
        
        \hline
        SNE 
        
        \cite{hinton2002stochastic} 
        
        Theorem \ref{thm:sne}
        & Gaussians on datapoints, $x_i$ \newline
        \(\displaystyle  \frac{\exp\left(-\|x_i - x_j\|^2 / 2\sigma_i^2\right)}{\sum_{k \neq i} \exp\left(-\|x_i - x_k\|^2 / 2\sigma_i^2\right)} \)
        & Gaussians on learned vectors, $\phi_i$ \newline
        \(\displaystyle \frac{\exp\left(-\|\phi_i - \phi_j\|^2\right)}{\sum_{k \neq i} \exp\left(-\|\phi_i - \phi_k\|^2\right)}\) \\ [2pt]
        
        \hline
        tSNE 
        
        \cite{van2008visualizing}
        
        Theorem \ref{thm:tsne}
        & Perplexity-sized Gaussians on datapoints, $x_i$ \newline
        \(\displaystyle \frac{\exp\left(-\|x_i -x_j\|^2 / 2\sigma_i^2\right)}{\sum_{k \neq i} \exp\left(-\|x_i - x_k\|^2 / 2\sigma_i^2\right)} \)
        & Cauchy distributions on learned vectors, $\phi_i$ \newline
        \(\displaystyle \frac{\left(1 + \|\phi_i - \phi_j\|^2\right)^{-1}}{\sum_{k \neq i} \left(1 + \|f\phi_i - \phi_k \|^2\right)^{-1}}\) \\ [2pt]
        
        \hline
        InfoNCE 
        
        \cite{bachman2019learning} 
        
        Theorem \ref{thm:infonce}
        & Uniform over positive pairs \newline
        \(\displaystyle \frac{1}{Z} \mathds{1}[i \text{ and } j \text{ are positive pairs }] \)
        & Gaussian based on deep features, $f_\phi(x_i)$ \newline
        \(\displaystyle\frac{\exp\left(-\|f_\phi(x_i) - f_\phi(x_j)\|^2\right)}{\sum_{k \neq i} \exp\left(-\|f_\phi(x_i) - f_\phi(x_k) \|^2\right)}\) \\ [2pt]
        
        \hline
        
        Triplet Loss 
        
          \cite{schroff2015facenet}
        
         Theorem \ref{thm:triplet_loss}
         & Uniform over positive pairs \newline
         \(\displaystyle \frac{1}{Z} \mathds{1}[i \text{ and } j \text{ are positive pairs }] \)
         & Gaussian based on deep features $f_\phi(x_i)$, with only one negative sample and $\sigma \rightarrow 0$   
          $\displaystyle\frac{\exp\left( - \| f_\phi(x_i) - f_\phi(x_j) \|^2/2\sigma^2 \right)}{\sum_{k \in \{i^+, i^-\}} \exp\left( - \| f_\phi(x_i) - f_\phi(x_k) \|^2 /2\sigma^2 \right)}$\\
        
        \hline
        
        PCA
        \cite{pearson1901liii} 
        
        Corollary \ref{thm:pca}
        & Indicator over the point itself \newline
         \(\displaystyle \mathds{1}[i = j] \)
        & Wide Gaussian on features based on a linear map $f_\phi(x_i)$ for $x_i$
          \(\displaystyle  \lim_{\sigma \to \infty}\frac{\exp\left(-\|\phi_i - \phi_j\|^2 / 2\sigma^2\right)}{\sum_{k \neq i} \exp\left(-\|\phi_i - \phi_k\|^2 / 2\sigma^2\right)}\)\\
        \hline  
        
        MDS
        
        \cite{kruskal1964multidimensional} 
        
        Theorem \ref{thm:mds}
        & Wide Gauss. on datapoints, $x_i$ \newline
        \(\displaystyle  \lim_{\sigma \to \infty} \frac{\exp\left(-\|x_i - x_j\|^2 / 2\sigma_i^2\right)}{\sum_{k \neq i} \exp\left(-\|x_i - x_k\|^2 / 2\sigma_i^2\right)} \)

        & Wide Gauss. on learned vectors., $\phi_i$$f_\phi(x_i)$ \newline
        \(\displaystyle  \lim_{\sigma \to \infty}\frac{\exp\left(-\|\phi_i - \phi_j\|^2 / 2\sigma^2\right)}{\sum_{k \neq i} \exp\left(-\|\phi_i - \phi_k\|^2 / 2\sigma^2\right)}\) \\

         \hline
        
        InfoNCE Clustering 
        
        (New in this work)
        % Theorem \ref{thm:infoncecluster}
        & Uniform over positive pairs \newline
        \(\displaystyle \frac{1}{Z} \mathds{1}[i \text{ and } j \text{ are positive pairs }] \)
        & Shared cluster likelihood by point \newline
        \( \displaystyle \frac{ f_\phi(x_i) \cdot  f_\phi(x_j)}{\mathbb{E}[\text{size of } x_i \text{'s cluster w.r.t } f_\phi ]} \) \\ [2pt]
        \hline
        SupCon 
        
        \cite{khosla2020supervised} 
        
        Theorem \ref{thm:supcon}
        & Uniform over classes \newline
        \(\displaystyle \frac{1}{Z} \mathds{1}[i \text{ and } j \text{ have the same class }] \)
        & Gaussian based on deep features, $f_\phi(x_i)$ \newline
        \(\displaystyle\frac{\exp\left(-\|f_\phi(x_i) - f_\phi(x_j)\|^2\right)}{\sum_{k \neq i} \exp\left(-\|f_\phi(x_i) - f_\phi(x_k) \|^2\right)}\) \\
      
        \hline
        Probabilistic k-Means 
        
        \cite{macqueen1967some}
        
        Theorem \ref{thm:kmeans}
        & Shared cluster likelihood by cluster \newline
        \(\displaystyle \sum_{c=1}^m \frac{p(f_\theta(x_i) \text{ and } f_\theta(x_j) \text{ are in cluster } c)}{\mathbb{E}[\text{size of cluster } c]} \)
        & Gaussians on Datapoints, $x_i$ \newline
        \(\displaystyle  \frac{\exp\left(-\|x_i - x_j\|^2 / 2\sigma_i^2\right)}{\sum_{k \neq i} \exp\left(-\|x_i - x_k\|^2 / 2\sigma_i^2\right)} \) \\
        \hline

        
        Normalized Cuts 
        
        \cite{shi2000normalized} 
        
        Theorem \ref{thm:normcuts}
        & Degree-weighted shared cluster likelihood by cluster \newline
        \(\displaystyle \sum_{c=1}^m \frac{p(f_\theta(x_i) \text{ and } f_\theta(x_j) \text{ are in cluster } c) \cdot d_j}{\mathbb{E}[\text{degree of members of cluster } c]} \)
        & Gaussians on edge weights \newline
        \( \displaystyle  \frac{\exp(w_{ij}/d_j)}{\sum_{k} \exp(w_{ik}/d_k)}\) \\ [2pt]        
        \hline

        

        Spectral Clustering
        
        \cite{ng2001spectral} 
        
        Theorem \ref{cor:spectral}
        & Shared cluster likelihood by cluster \newline
        \(\displaystyle \sum_{c=1}^m \frac{p(f_\theta(x_i) \text{ and } f_\theta(x_j) \text{ are in cluster } c)}{\mathbb{E}[\text{size of cluster } c]} \)
        & Gaussians on Spectral Embeddings, $x_i$ \newline
        \(\displaystyle  \frac{\exp\left(-\|x_i - x_j\|^2 / 2\sigma_i^2\right)}{\sum_{k \neq i} \exp\left(-\|x_i - x_k\|^2 / 2\sigma_i^2\right)} \) \\ [2pt]
        
        \hline
        
        Mutual Info. Clust.
        
        \cite{adaloglou2023exploring} 
        
        Theorem \ref{thm:pmi}
        & Uniform over nearest neighbors \newline
        \(\displaystyle \frac{1}{k} \mathds{1}[j \text{ is a k-nearest neighbor of } i ] \)
        & Shared cluster likelihood by cluster \newline
        \(\displaystyle \sum_{c=1}^m \frac{p(f_\phi(x_i) \text{ and } f_\phi(x_j) \text{ are in cluster } c)}{\mathbb{E}[\text{size of cluster } c]} \) \\ [2pt]     
        \hline
        CMC \& CLIP 
        
        \cite{tian2020contrastive}
        
        Theorem \ref{thm:cmc}
        & Uniform over positive pairs from different modalities $V$ \newline
        \(\displaystyle \frac{1}{Z} \mathds{1}[i \text{ and } j \text{ are positive pairs and } V_i \neq V_j] \)
        & Gaussian based on deep features, $f_\phi(x_i)$ \newline
        \(\displaystyle\frac{\exp\left(-\|f_\phi(x_i) - f_\phi(x_j)\|^2\right)}{\sum_{k \in V_j} \exp\left(-\|f_\phi(x_i) - f_\phi(x_k) \|^2\right)}\) \\ [2pt]
        
        \hline
        Cross Entropy
        
        \cite{good1963maximum}
        
        Corollary  \ref{thm:ce}
        
        & Indicator function over Labels \newline
        \(\displaystyle \frac{1}{|C|} \mathds{1}[i \in D \text{ is a data point in a class }j \in C] \)
        & Gaussian based on deep features \newline
        \(\displaystyle\frac{\exp\left(f_\phi(x_i) \cdot \phi_j \right)}{\sum_{k \in C} \exp\left(f_\phi(x_i) \cdot \phi_k\right)} \) \\ [2pt]

        \hline
        
        Masked Lang. Modeling

\cite{devlin2019bertpretrainingdeepbidirectional}

        Corollary  \ref{thm:mlm}
        
        & Empirical dist. over contexts, $i$, and tokens, $j$ \newline
        \(\displaystyle \frac{1}{Z} \#[\text{Context } i \text{ precedes token }j] \)
        & Gaussian based on deep features $f_\phi(x_i)$, and token embeddings,  $\phi_j$ \newline
        \(\displaystyle\frac{\exp\left(f_\phi(x_i) \cdot \phi_j \right)}{\sum_{k \in C} \exp\left(f_\phi(x_i) \cdot \phi_k\right)} \) \\ [2pt]
        
%        \hline
%        
%        Reconstruction Loss
%        Theorem \ref{thm:mse}
%        & Dirac Delta over target \( y_i \) for all real \(y \in \mathbb{R}^n\) \newline
%        \( \delta(y - y_i) \) & Continuous Gaussian centered at \( f_\phi(x_i) \) \newline
%        \(\displaystyle \propto \exp\left( -{\|y - f_\phi(x_i)\|^2}/{2\sigma^2} \right) \) \\
        \hline  
    \end{tabular}
    }

    \caption{\textbf{I-Con unifies representation learners} under different choices of $p_\theta(j|i)$ and $q_\phi(j|i)$. Proofs of the propositions in this table can be found in the supplement. }
    \label{tab:choice_pq}
\end{table}

==> sections/table_merged.tex <==
\begin{table}[p]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{8pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|>{\centering\arraybackslash}p{2.7cm}
                |>{\centering\arraybackslash}p{5.8cm}
                |>{\centering\arraybackslash}p{5.9cm}|} 
\rowcolor{lightgray!50}
\hline
\textbf{Method} & \textbf{Choice of $p_\theta(j \mid i)$} & \textbf{Choice of $q_\phi(j \mid i)$} \\[3pt]
\hline
%-----------------------------------------------------------------------------------------
% 1) PCA
\multirow{2}{*}{\parbox{2.7cm}{\centering \textbf{PCA}\\[4pt]\cite{pearson1901liii}\\Corollary \ref{thm:pca}}}
 & Indicator over the point itself 
   \[
     \mathds{1}[\,i = j\,]
   \]
 & \parbox{5.9cm}{\centering 
    Wide Gaussian on linear features  
    \[
      \lim_{\sigma \to \infty}
      \frac{\exp\!\bigl(-\|\phi_i - \phi_j\|^2 / 2\sigma^2\bigr)}
           {\sum_{k \neq i} \exp\!\bigl(-\|\phi_i - \phi_k\|^2 / 2\sigma^2\bigr)}
    \]
 } \\
\hline
%-----------------------------------------------------------------------------------------
% 2) SNE
\multirow{2}{*}{\parbox{2.7cm}{\centering \textbf{SNE}\\[4pt]\cite{hinton2002stochastic}\\Theorem \ref{thm:sne}}}
 & Gaussians on datapoints, $x_i$ 
   \[
     \frac{\exp\!\bigl(-\|x_i - x_j\|^2 / 2\sigma_i^2\bigr)}
          {\sum_{k \neq i}\exp\!\bigl(-\|x_i - x_k\|^2 / 2\sigma_i^2\bigr)}
   \]
 & Gaussians on learned vectors, $\phi_i$ 
   \[
     \frac{\exp\!\bigl(-\|\phi_i - \phi_j\|^2\bigr)}
          {\sum_{k \neq i} \exp\!\bigl(-\|\phi_i - \phi_k\|^2\bigr)}
   \]
 \\
\hline
%-----------------------------------------------------------------------------------------
% 3) t-SNE
\multirow{2}{*}{\parbox{2.7cm}{\centering \textbf{t-SNE}\\[4pt]\cite{van2008visualizing}\\Theorem \ref{thm:tsne}}}
 & Perplexity-sized Gaussians on datapoints, $x_i$ 
   \[
     \frac{\exp\!\bigl(-\|x_i - x_j\|^2 / 2\sigma_i^2\bigr)}
          {\sum_{k \neq i}\exp\!\bigl(-\|x_i - x_k\|^2 / 2\sigma_i^2\bigr)}
   \]
 & Cauchy distributions on learned vectors, $\phi_i$ 
   \[
     \frac{\bigl(1 + \|\phi_i - \phi_j\|^2\bigr)^{-1}}
          {\sum_{k \neq i}\bigl(1 + \|\phi_i - \phi_k\|^2\bigr)^{-1}}
   \]
 \\
\hline
%-----------------------------------------------------------------------------------------
% (4-7) MERGED p_\theta: InfoNCE, Triplet, InfoNCE Clust, t-SimCLR/t-SimCNE
\multirow{4}{*}{\parbox{2.7cm}{\centering 
\textbf{InfoNCE}\\[2pt]\cite{bachman2019learning}\\Theorem \ref{thm:infonce} 
\\[6pt]
\textbf{Triplet Loss}\\[2pt]\cite{schroff2015facenet}\\Theorem \ref{thm:triplet_loss} 
\\[6pt]
\textbf{InfoNCE Clustering}\\(New in this work)
\\[6pt]
\textbf{t-SimCLR and t-SimCNE}
}} 
 & \multirow{4}{*}{\parbox{5.8cm}{\centering
 \textbf{All share the same:} \\[4pt]
 \(\displaystyle 
   \frac{1}{Z}\,\mathds{1}\bigl[\text{$i$ and $j$ are positive pairs}\bigr]
 \)
 }}
 & \parbox{5.9cm}{\centering
   \underline{\textbf{InfoNCE}}: Gaussian on deep features 
   \[
     \frac{\exp\!\bigl(-\|f_\phi(x_i) - f_\phi(x_j)\|^2\bigr)}
          {\sum_{k \neq i}\exp\!\bigl(-\|f_\phi(x_i) - f_\phi(x_k)\|^2\bigr)}
   \]
 }
\\ \cline{3-3}
 & & \parbox{5.9cm}{\centering
   \underline{\textbf{Triplet Loss}}: Gaussian on deep features (1 neg. sample, $\sigma\to 0$)
   \[
     \frac{\exp\!\bigl(-\|f_\phi(x_i) - f_\phi(x_j)\|^2/2\sigma^2\bigr)}
          {\sum_{k\in\{i^+,\,i^-\}}
           \exp\!\bigl(-\|f_\phi(x_i) - f_\phi(x_k)\|^2/2\sigma^2\bigr)}
   \]
 }
\\ \cline{3-3}
 & & \parbox{5.9cm}{\centering
   \underline{\textbf{InfoNCE Clustering}}: shared cluster likelihood
   \[
     \frac{\,f_\phi(x_i) \cdot f_\phi(x_j)\,}%
          {\mathbb{E}[\text{size of $x_i$'s cluster}]}
   \]
 }
\\ \cline{3-3}
 & & \parbox{5.9cm}{\centering
   \underline{\textbf{t-SimCLR / t-SimCNE}}: Cauchy on learned vectors
   \[
     \frac{\bigl(1 + \|\phi_i - \phi_j\|^2\bigr)^{-1}}
          {\sum_{k \neq i} \bigl(1 + \|\phi_i - \phi_k\|^2\bigr)^{-1}}
   \]
 }
\\
\hline
%-----------------------------------------------------------------------------------------
% 8) SupCon
\multirow{2}{*}{\parbox{2.7cm}{\centering \textbf{SupCon}\\[2pt]\cite{khosla2020supervised}\\Theorem \ref{thm:supcon}}}
 & Uniform over classes 
   \[
     \frac{1}{Z}\,\mathds{1}[\text{$i$ and $j$ have same class}]
   \]
 & Gaussian on deep features 
   \[
     \frac{\exp\!\bigl(-\|f_\phi(x_i) - f_\phi(x_j)\|^2\bigr)}
          {\sum_{k \neq i}\exp\!\bigl(-\|f_\phi(x_i) - f_\phi(x_k)\|^2\bigr)}
   \]
\\
\hline
%-----------------------------------------------------------------------------------------
% 9) X-Sample
\multirow{2}{*}{\parbox{2.7cm}{\centering \textbf{X-Sample}}}
 & Gaussians on features (e.g.\ caption embeddings) $x_i$
   \[
     \frac{\exp\!\bigl(-\|x_i - x_j\|^2 / 2\sigma_i^2\bigr)}
          {\sum_{k \neq i}\exp\!\bigl(-\|x_i - x_k\|^2 / 2\sigma_i^2\bigr)}
   \]
 & Gaussian on deep features
   \[
     \frac{\exp\!\bigl(-\|f_\phi(x_i) - f_\phi(x_j)\|^2\bigr)}
          {\sum_{k \neq i}\exp\!\bigl(-\|f_\phi(x_i) - f_\phi(x_k)\|^2\bigr)}
   \]
\\
\hline
%-----------------------------------------------------------------------------------------
% 10) CMC & CLIP
\multirow{2}{*}{\parbox{2.7cm}{\centering \textbf{CMC \& CLIP}\\[2pt]\cite{tian2020contrastive}\\Theorem \ref{thm:cmc}}}
 & Uniform over positive pairs (different modalities)
   \[
     \frac{1}{Z}\,\mathds{1}[\text{$i$ and $j$ are pos. pairs, }V_i\neq V_j]
   \]
 & Gaussian on deep features 
   \[
     \frac{\exp\!\bigl(-\|f_\phi(x_i)-f_\phi(x_j)\|^2\bigr)}
          {\sum_{k \in V_j}\exp\!\bigl(-\|f_\phi(x_i)-f_\phi(x_k)\|^2\bigr)}
   \]
\\
\hline
%-----------------------------------------------------------------------------------------
% 11-12) Prob k-Means & Spectral Clustering (MERGE p_\theta)
\multirow{2}{*}{\parbox{2.7cm}{\centering 
\textbf{Probabilistic k-Means}\\[2pt]\cite{macqueen1967some}\\Theorem \ref{thm:kmeans}
\\[6pt]
\textbf{Spectral Clustering}\\[2pt]\cite{ng2001spectral}\\Theorem \ref{cor:spectral}
}}
 & \multirow{2}{*}{\parbox{5.8cm}{\centering
 \textbf{Both: Shared cluster likelihood}
 \[
   \sum_{c=1}^m 
   \frac{p\!\bigl(f_\theta(x_i)\text{ and }f_\theta(x_j)\text{ in cluster } c\bigr)}
        {\mathbb{E}[\text{size of cluster } c]}
 \]
}}
 & \parbox{5.9cm}{\centering
   \underline{\textbf{Prob. k-Means}}: Gaussians on datapoints
   \[
     \frac{\exp\!\bigl(-\|x_i - x_j\|^2/2\sigma_i^2\bigr)}
          {\sum_{k \neq i}\exp\!\bigl(-\|x_i - x_k\|^2/2\sigma_i^2\bigr)}
   \]
 }
\\ \cline{3-3}
 & & \parbox{5.9cm}{\centering
   \underline{\textbf{Spectral Clustering}}: Gaussians on spectral embeddings
   \[
     \frac{\exp\!\bigl(-\|x_i - x_j\|^2/2\sigma_i^2\bigr)}
          {\sum_{k \neq i}\exp\!\bigl(-\|x_i - x_k\|^2/2\sigma_i^2\bigr)}
   \]
 }
\\
\hline
%-----------------------------------------------------------------------------------------
% 13) Normalized Cuts
\multirow{2}{*}{\parbox{2.7cm}{\centering \textbf{Normalized Cuts}\\[2pt]\cite{shi2000normalized}\\Theorem \ref{thm:normcuts}}}
 & Degree-weighted shared cluster likelihood
   \[
     \sum_{c=1}^m \!\!
     \frac{p\!\bigl(f_\theta(x_i)\text{ and }f_\theta(x_j)\text{ in clust }c\bigr)\cdot d_j}
          {\mathbb{E}[\text{degree of cluster } c]}
   \]
 & Gaussians on edge weights 
   \[
     \frac{\exp\!\bigl(w_{ij}/d_j\bigr)}
          {\sum_{k}\exp\!\bigl(w_{ik}/d_k\bigr)}
   \]
\\
\hline
%-----------------------------------------------------------------------------------------
% 14) Mutual Info. Clustering
\multirow{2}{*}{\parbox{2.7cm}{\centering \textbf{Mutual Info. Clust.}\\[2pt]\cite{adaloglou2023exploring}\\Theorem \ref{thm:pmi}}}
 & Uniform over nearest neighbors
   \[
     \frac{1}{k}\,\mathds{1}[\text{$j$ is $k$-NN of $i$}]
   \]
 & Shared cluster likelihood 
   \[
     \sum_{c=1}^m 
       \frac{p\!\bigl(f_\phi(x_i)\text{ and }f_\phi(x_j)\text{ in clust }c\bigr)}
            {\mathbb{E}[\text{size of cluster }c]}
   \]
\\
\hline
%-----------------------------------------------------------------------------------------
% 15-16) Cross Entropy & Harmonic-Loss (MERGE p_\theta)
\multirow{2}{*}{\parbox{2.7cm}{\centering 
\textbf{Cross Entropy}\\[2pt]\cite{good1963maximum}\\Corollary \ref{thm:ce}
\\[6pt]
\textbf{Harmonic-Loss}\\[2pt]\cite{good1963maximum}\\Corollary \ref{thm:ce}
}}
 & \multirow{2}{*}{\parbox{5.8cm}{\centering
 \textbf{Both: Indicator function over labels}
 \[
   \frac{1}{|C|}\,\mathds{1}\bigl[\text{$i$ in data set of class $j$}\bigr]
 \]
}}
 & \parbox{5.9cm}{\centering
   \underline{\textbf{Cross Entropy}}: softmax on deep features
   \[
     \frac{\exp\!\bigl(f_\phi(x_i)\cdot\phi_j\bigr)}
          {\sum_{k \in C}\exp\!\bigl(f_\phi(x_i)\cdot\phi_k\bigr)}
   \]
 }
\\ \cline{3-3}
 & & \parbox{5.9cm}{\centering
   \underline{\textbf{Harmonic-Loss}}: student-$t$ type softmax
   \[
     \frac{\exp\!\bigl(f_\phi(x_i)\cdot\phi_j\bigr)}
          {\sum_{k \in C}\exp\!\bigl(f_\phi(x_i)\cdot\phi_k\bigr)}
   \]
 }
\\
\hline
%-----------------------------------------------------------------------------------------
% 17) Masked LM
\multirow{2}{*}{\parbox{2.7cm}{\centering \textbf{Masked Lang. Modeling}\\[4pt]\cite{devlin2019bertpretrainingdeepbidirectional}\\Corollary \ref{thm:mlm}}}
 & Empirical dist.\ over context/token
   \[
     \frac{1}{Z}\,\#\bigl[\text{Context $i$ precedes token $j$}\bigr]
   \]
 & Softmax on deep context and token embeddings
   \[
     \frac{\exp\!\bigl(f_\phi(x_i)\cdot\phi_j\bigr)}
          {\sum_{k \in C}\exp\!\bigl(f_\phi(x_i)\cdot\phi_k\bigr)}
   \]
\\
\hline
%-----------------------------------------------------------------------------------------
\end{tabular}
}
\caption{\textbf{An example of a reorganized table} that groups methods with identical $p_\theta(j|i)$ or $q_\phi(j|i)$ and merges their cells. Citations/theorem references have been placed on separate lines for clarity.}
\label{tab:merged_choice_pq}
\end{table}

